Strong existence and uniqueness of the tilt-indexed Busemann process in the planar corner growth model

We show that the Busemann process indexed by tilts in the super-differential of the limit shape exists and is unique in the strong sense in the i.i.d.\ planar corner growth model. This means that every probability space that supports the field of i.i.d.~weights supports a copy of the process and any two realizations of the process are equal almost surely.

==> LPPBuseProcMacros.tex <==
%This is the one in CFT/Shox2 overleaf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages go here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bbfamily}{\fontencoding{U}\fontfamily{bbold}\selectfont}
\DeclareMathAlphabet{\mathbbold}{U}{bbold}{m}{n}

\usepackage{amsmath,amsfonts,amsthm,xcolor,amssymb,mathrsfs,pgfplots,enumitem,comment}   %F: enumitem is better than enumerate
%%% types of  labels:  [label=(roman*)]  \arabic*  \alph*    also under \itemize can use different symbols to mark items
  
\RequirePackage[colorlinks,urlcolor=my-blue,linkcolor=my-red,citecolor=my-green]{hyperref}

\usepackage[numbers,comma,square,sort&compress]{natbib}
\usepackage{xargs}
\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize]{todonotes}
\usepackage{pdfcomment}
\usepackage{mathdots} 
\usepackage{bm}
\usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work  
\usepackage{hyphenat}
\usepackage[utf8]{inputenc}
%\usepackage[notref,notcite]{showkeys}
%%%%  2019-03-22 Timo moved showkeys into the latex file itself in order to toggle it for printing. 
\usepackage{caption}
\usepackage{subcaption}
%\usepackage{a4wide}
\usepackage{accents}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,decorations.markings,shapes.misc}
\usepackage{graphicx}
\usepackage{chngcntr}
\usepackage{float} %needed to fix the figures

\usepackage{rotating,centernot,cancel}    %% to manipulate symbols (Timo 2019-03-25) 
\usepackage[normalem]{ulem}   %%% needed for \sout  

\numberwithin{figure}{section}
\numberwithin{equation}{section}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New macros for this paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%General
\tikzset{middlearrow/.style={
        decoration={markings,
            mark= at position 0.6 with {\arrow{#1}} ,
        },
        postaction={decorate}
    }
}

\newcommand\aUset{\sV^{\,\w}} %The set of directions on which non-coalescence holds
\newcommand\gpp{g_{\text{pp}}} %The shape function
\newcommand\shape{\textup{g}}
\newcommand\gpl{g_{\text{pl}}} %The pl shape
%\newcommand\gpp{g} %The shape function without pp subscript 
\newcommand\dgpp[1]{\widecheck{g}_{\text{pp}}^{#1}} %The shape function
\def\gppa{\gamma}   %% this is from the 2017 cocycle paper 

\def\gppU{\varphi}  %% an auxiliary function, generic notation  

\newcommand\T{T} %The shift, T
\def\shift{T}
\def\shifthat{\wh\shift} 
%\newcommand\cif{\xi_*} %The competition interface random variable
%\newcommand\cid{\xi_*} %The competition interface random variable
\newcommand\adir{\zeta} 
\newcommand\wchk[1]{\widecheck{\omega}^{#1}} %Dual weights

%Busemann functions
\newcommand\B[1]{B^{#1}} %The Busemann function
\newcommand\BBbar[1]{{\overline B}^{#1}} %The Busemann function
\newcommand\Ubar{\overline U} %The Busemann function
\newcommand\dB[1]{u^{#1}} %The Busemann function
\newcommand\dBbar[1]{\overline{u}^{#1}} %The Busemann function

%Geodesics
\def\geobus{{\mathbf x}} %Busemann geodesic
\newcommand\geo[3]{\boldsymbol{\gamma}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
\newcommand\geobar[3]{{\overline{\boldsymbol{\gamma}}}_{#1}^{\,#2,#3}} %Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction
\newcommand\fgeod[1]{\sigma_{#1}} %A finite rightmost geodesic. The argument is the index.
\newcommand\cgeod[1]{\phi_{#1}} %The geodesic generated by a cocycle generated by a geodesic.
\newcommand\cDLR{\Phi}
\newcommand\QDLR{Q^{\mathrm{DLR}}}
\newcommand\dgeod[1]{\psi_{#1}} %The geodesic Busemann process geodesic
\newcommand\geod[1]{\pi_{#1}} %A generic geodesic without a root or direction. The argument is the index.
\newcommand\geodbar[1]{{\overline\pi}_{#1}} %A generic geodesic without a root or direction. The argument is the index.
\newcommand\geodd[1]{\rho_{#1}} %Another generic geodesic without a root or direction. 
\newcommand\geoddbar[1]{{\overline\rho}_{#1}} %Another generic geodesic without a root or direction. 
\newcommand\geoddd[1]{\gamma_{#1}} %Another generic geodesic without a root or direction. 
\newcommand\geodddd[1]{\lambda{#1}} %Another generic geodesic without a root or direction. 
%\newcommand\geod[1]{\boldsymbol{\gamma }_{#1}} %A generic geodesic without a root or direction. The argument is the index.
\newcommand\geodhat[1]{{\wh\pi}_{#1}} % geodesic defined on the bigger space 
\newcommand\geoddhat[1]{\wh\rho_{#1}} % 
\newcommand\cgeo{\pi} %a random coalescing geodesic
\newcommand\gap[2]{D^{#1}_{#2}}   %% D^{stub}_{vertex on geodesic}  

\def\geodf{\sigma}  %% finite geodesic, w/o arguments 
\def\geoddf{\tau}  %% finite geodesic, w/o arguments 
\def\geodddf{\lambda}  %% finite geodesic, w/o arguments 
\newcommand\rmgeod[2]{\boldsymbol{\rho}^{#1}_{#2}}
\newcommand\lmgeod[2]{\boldsymbol{\lambda}^{#1}_{#2}}
\newcommand\cilgeod[2]{\boldsymbol{\gamma}^{#1,-}_{#2}}
\newcommand\cirgeod[2]{\boldsymbol{\gamma}^{#1,+}_{#2}}
\newcommand\geogeod[2]{{}^{#1}\!\psi^{#2}}
\def\cif{\varphi}

\newcommand\bfrho{{\boldsymbol{\rho}}}
\newcommand\bfrhol{\underline{\boldsymbol{\rho}}}
\newcommand\bfrhor{\overline{\boldsymbol{\rho}}}
\newcommand\bflambda{{\boldsymbol{\lambda}}}
\newcommand\bflaml{\underline{\boldsymbol{\lambda}}}
\newcommand\bflamr{\overline{\boldsymbol{\lambda}}}
\newcommand\bfgamma{{\boldsymbol{\gamma}}}
\newcommand\bfpi{{\boldsymbol{\pi}}}

\newcommand\invAL{\alpha}   %value of A - L of a path   


\def\selongarrow{\ \tikz{\draw[->] (0,0.15) -- (1,0);}\ }

\newcommand\alphabar{\overline\alpha}
\newcommand\labd{\lab^{\scaleobj{0.8}{(d)}}}
\newcommand\whlabd{\wh\lab^{\scaleobj{0.8}{(d)}}}
\newcommand\labddet{\labdet^{\scaleobj{0.8}{(d)}}}
\newcommand\labinf{\underline\kappa}
\newcommand\labsup{\overline\kappa}
\newcommand\lab{\kappa} %the label of a geodesic
\newcommand\labdet{{\boldsymbol{\lab}}} %the deterministic version of the label of a geodesic
\newcommand\labinfdet{{\underline{\boldsymbol{\lab}}}} 
\newcommand\labsupdet{{\overline{\boldsymbol{\lab}}}}
\newcommand\ulab{\underline\kappa} %the label of a geodesic
\newcommand\olab{\overline\kappa} %the label of a geodesic

%\newcommand\kSfor[1]{\kS^{\not<#1}}
\newcommand\kSforfor[1]{\kS^+_{#1}}
\newcommand\kSfor{\kS^+}
\newcommand\kSforbar{{\overline\kS}^+}
\newcommand\sFforbar{{\overline\sF}^+}
\newcommand\sFfor{\sF^{+}}
\newcommand\kSbac{\kS^{-}}
\newcommand\tail{\mathfrak T}

\newcommand\swgeo[3]{\boldsymbol{\sigma}_{#1}^{\,#2,\tspa#3}} %SW Geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction

\newcommand\dgeo[3]{\boldsymbol{\gamma}_{#1}^{*,\,#2\!,\,#3}} %dual geodesic. Arguments are 1.) the index, 2.) the starting point, 3.) the direction


\newcommand\geob[3]{\boldsymbol{\rho}_{#1}^{\,#2,\tspa#3}} %Another Geodesic. Arguments are 1.) the index, 2.3.) some symbol, incl.  the starting point, 



%Coalescence points
%\newcommand\coal[1]{\mathbf{z}^{#1}} %Coalescence point. The argument is the direction.

%Split points
\newcommand\spt[2]{s_{#1}(#2)}


%The geodesic graphs and vertex sets 
\newcommand\G[1]{\mathcal{G}_{#1}} %The graph of geodesics. Argument is the direction.
\newcommand \dG[1]{\mathcal{G}^*_{#1}} %The dual graph to the graph of geodesics. Argument is the direction.
\newcommand\dGpp[1]{\widecheck{G}^{#1}} %The dual passage times
%\newcommand\dS[1]{\mathcal{T}_{#1}^{*}}
\newcommand\dS[1]{\mathcal{G}_{\cup#1}^{*}}   %% trying out another option
\newcommand\Geo{\cG}
\makeatletter
\newcommand{\raisemath}[1]{\mathpalette{\raisem@th{#1}}}
\newcommand{\raisem@th}[3]{\raisebox{#1}{$#2#3$}}
\makeatother
\newcommand\Geoint{{}^{\raisemath{1pt}{o}}\hspace{-0.15em}\cG}
\newcommand\Geobar{\overline\Geo}
\newcommand\RIGeow{\cG^{{\rm ri},\w}}
\newcommand\Geocons[1]{\cG^{\mathrm{cons},#1}}

\def\Shock#1#2{{\bfS}^{#1}_{#2}}
\def\shock#1{{\bfS}_{#1}^*}      %%%% red points 
\def\ans#1#2{{\bfA}_{#1}^*(#2)}    %%%% ancestors 
\def\shockG#1{{\mathcal S}_{#1}^*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros inherited from the DLR paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\addtolength{\hoffset}{-.8in} 
%\addtolength{\textwidth}{1.6in}
%\addtolength{\voffset}{-.3in} 
%\addtolength{\footskip}{.3in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\evensidemargin}{0in}
%\setlength{\footskip}{0.2in}
%\setlength{\topmargin}{0.5in}
%\addtolength{\textheight}{.7in}
%\baselineskip=12pt   %%seems to make no difference? 
%\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1


%\RequirePackage{xcolor}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\definecolor{really-light-gray}{gray}{0.8}
\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
\definecolor{nicosred}{rgb}{0.65,0.1,0.1}
\definecolor{light-gray}{gray}{0.7}

\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}

\addtolength\marginparwidth{0.35in}

\newcommandx{\addmath}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\fixtext}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\note}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{#2}}

%\pgfplotsset{compat=newest}
%\pgfplotsset{plot coordinates/math parser=false}
%\newlength\figureheight
%\newlength\figurewidth

%%%%%%   Symbols for plus and minus 
%\newcommand{\sig}{{\mbox{\larger$\square$}}}
%\newcommand{\gis}{\boxminus}
%\newcommand{\sig}{\boxempty}   % too large 
\newcommand{\sig}{{\scaleobj{0.8}{\boxempty}}} 
\newcommand{\sigg}{{\scaleobj{0.9}{\boxempty}}} 
%\newcommand{\sig}{{\raisebox{1pt}{\scaleobj{0.8}{\boxempty}}}}  
\newcommand{\gis}{{\raisebox{1pt}{\scaleobj{0.6}{\boxslash}}}}   
\newcommand{\giss}{{\raisebox{1pt}{\scaleobj{0.8}{\boxslash}}}}   
%\newcommand{\gis}{{\mbox{\larger$\diamond$}}}
%\newcommand{\sig}{\square}
%%%%    Try out also \ovoid and \ominus

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

%bold face
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}


\newcommand{\mfa}{\mathfrak{a}}
\newcommand{\mfb}{\mathfrak{b}}
\newcommand{\mfc}{\mathfrak{c}}
\newcommand{\mfd}{\mathfrak{d}}
\newcommand{\mfe}{\mathfrak{e}}
\newcommand{\mff}{\mathfrak{f}}
\newcommand{\mfg}{\mathfrak{g}}
\newcommand{\mfh}{\mathfrak{h}}
\newcommand{\mfi}{\mathfrak{i}}
\newcommand{\mfj}{\mathfrak{j}}
\newcommand{\mfk}{\mathfrak{k}}
\newcommand{\mfl}{\mathfrak{l}}
\newcommand{\mfm}{\mathfrak{m}}
\newcommand{\mfn}{\mathfrak{n}}
\newcommand{\mfo}{\mathfrak{o}}
\newcommand{\mfp}{\mathfrak{p}}
\newcommand{\mfq}{\mathfrak{q}}
\newcommand{\mfr}{\mathfrak{r}}
\newcommand{\mfs}{\mathfrak{s}}
\newcommand{\mft}{\mathfrak{t}}
\newcommand{\mfu}{\mathfrak{u}}
\newcommand{\mfv}{\mathfrak{v}}
\newcommand{\mfw}{\mathfrak{w}}
\newcommand{\mfx}{\mathfrak{x}}
\newcommand{\mfy}{\mathfrak{y}}
\newcommand{\mfz}{\mathfrak{z}}


\newcommand{\mfG}{\mathfrak{G}}
\newcommand{\mfS}{\mathfrak{S}}
\newcommand{\kS}{\mathfrak{S}}
\newcommand{\kShat}{\widehat{\mathfrak{S}}}

%script
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\sD}{\mathcal{D}}
\newcommand{\sE}{\mathcal{E}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sG}{\mathcal{G}}
\newcommand{\sH}{\mathcal{H}}
\newcommand{\sI}{\mathcal{I}}
\newcommand{\sJ}{\mathcal{J}}
\newcommand{\sK}{\mathcal{K}}
\newcommand{\sL}{\mathcal{L}}
\newcommand{\sM}{\mathcal{M}}
\newcommand{\sN}{\mathcal{N}}
\newcommand{\sO}{\mathcal{O}}
\newcommand{\sP}{\mathcal{P}}
\newcommand{\sQ}{\mathcal{Q}}
\newcommand{\sR}{\mathcal{R}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sT}{\mathcal{T}}
\newcommand{\sU}{\mathcal{U}}
\newcommand{\sV}{\mathcal{V}}
\newcommand{\sW}{\mathcal{W}}
\newcommand{\sX}{\mathcal{X}}
\newcommand{\sY}{\mathcal{Y}}
\newcommand{\sZ}{\mathcal{Z}}

\font \mymathbb = bbold10 at 11pt
\newcommand{\one}{\mbox{\mymathbb{1}}}
%\newcommand{\one}{\mathbf{1}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\supp}{supp}

\def\hmin{h_{\min}}
\def\hmax{h_{\max}}

\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\range{\mathcal R}
\def\Uset{\mathcal U}
\def\Aset{{\mathbf M}^{\lab,\w}}
\def\Asetd{{\mathbf M}^{\labd\!,\,\w}}
\def\Asetwtil{\mathbf M^{\lab,\wt\w}}
\def\Asetwg{\mathbf M^{\lab,\w(\wg)}}
\def\Asethat{\mathbf M^{\lab,\what}}
\def\AsetTuhat{\mathbf M^{\lab,\That_u\what}}
\def\Asetwgtil{\mathbf M^{\lab,\w(\wgtil)}}
\def\AsetTu{\mathbf M^{\lab,T_u\w}}
\def\detAset{{\mathcal M}^{\lab}}
\def\detAsetR{{\mathcal M}^{R\lab}}
\def\detAsetd{{\mathcal M}^{\labd}}
\def\Adense{{\mathcal A}^{\lab}_0}
\def\Addense{{\mathcal A}^{\labd}_0}
\def\uAset{{\mathbf M}^{\ulab,\w}}
\def\detuAset{{\mathcal M}^{\ulab}}
\def\cKcoal{\mathcal K_c}
\def\cKhatcoal{\widehat{\mathcal{K}}_c}
\def\cKhatcoalfor{\widehat{\mathcal{K}}_c^+}
\def\cKhatfor{\widehat{\mathcal{K}}^+}
%\def\cKhatforerg{\widehat{\mathcal K}_{\Gcc,e}^+}
\def\cKGcc{\mathcal K_\Gcc}
\def\cKhatGcchat{\widehat{\mathcal K}_{\Gcchat}}
\def\cKhaterg{\widehat{\mathcal K}_{\Gcchat,e}}
\def\cKfor{\mathcal K^+}
\def\cKcoalfor{\mathcal K_c^+}
\def\cHerg{\mathcal H_e}
\def\cHfor{\mathcal H^+}
\def\cHcoal{\mathcal H_c}
\def\cHcoalfor{\mathcal H_c^+}
\def\cH{\mathcal H}
\def\cHdense{\mathcal H_0}
\def\cHGcc{\mathcal H_\Gcc}
\def\Bruno{\mathcal A^\w}
\def\Gcc{{{\mathbbold\Pi}_c}}
\def\Gcchat{{\wh{\mathbbold\Pi}_c}}
\def\Gccfor{{\mathbbold\Pi^+_c}}
\def\fUset{\mathcal H}   % remove flat parts from \ri\Uset 
\newcommand{\dUset}[1]{\widecheck{\mathcal U}^{#1}}
%\def\Usetnice{\Uset_1}
\def\Usetnonuniq{\Uset_x^\w}
\def\Usetnonuniqz{\Uset_0^\w}
\def\Udense{\Uset_0}
\def\Ddense{\Diff_0}
\def\Usetnonuniqhat{\Uset_x^\what}
%\def\riUset{\Uset^\circ}

\def\preceqas{\preceq_{\mathrm{as}}}
\def\precneqas{\precneq_{\mathrm{as}}}
\def\succeqas{\succeq_{\mathrm{as}}}
\def\succneqas{\succneq_{\mathrm{as}}}

\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}

\newcommand{\e}{\varepsilon}
\def\Diff{\sD}
\def\Cont{\sC}
\def\w{\omega}
\def\wbar{{\bar\w}}
\def\wtil{{\widetilde\w}}
\newcommand{\ehat}{\widehat{e}}
\newcommand{\et}{\widehat{e}_1}   % e_1 + e_2 
\newcommand{\etstar}{\et^{\,*}}   %   (e_1 + e_2 )/2 
\newcommand{\ex}{\widehat{e}_2}   % e_2 - e_1 
\newcommand{\exstar}{\ex^{\,*}}   % (e_2 - e_1)/2  
\def\unif{\vartheta}
\def\Unif{\Gamma}
\def\eB{\kappa}
\def\EB{\cK}
\def\Bavg{\overline B}
\def\Bhat{{\widehat B}}
\def\Ahat{{\widehat A}}
\def\Gbar{\overline G}
\providecommand{\abs}[1]{\vert#1\vert}
\providecommand{\babs}[1]{\bigl\vert#1\bigr\vert}
\providecommand{\Babs}[1]{\Bigl\vert#1\Bigr\vert}
\providecommand{\norm}[1]{\Vert#1\Vert}
\providecommand{\bnorm}[1]{\bigl\Vert#1\bigr\Vert}

\def\what{{\widehat\w}}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\Omhat{\widehat\Omega}
\def\Ombar{\overline\Omega}
\def\Omerg{\Omega^{\mathrm{???}}}
\def\Omreg{\Omega^{\mathrm{reg}}}
\def\Omjump{\Omega^{\mathrm{jump}}_0}
\def\OmCou{\Omega^{\mathrm{no3geo}}_0}
\def\Ombiinf{\Omega^{\mathrm{nobi}}_0}
\def\Omregjump{\Omega_0^{\mathrm{reg,jump}}}
\def\ddd{\displaystyle}
\def\fe{\Lambda}
\def\fepl{\fe_{\rm{pl}}}
\def\Zne{Z^{\rm NE}} 
\def\Qne{Q^{\rm NE}} 
\def\Zn{Z^{\rm N}} 
\def\xibar{\bar\xi}
\def\Abar{\overline A}
\def\zetabar{\bar\zeta}
\def\etabar{\bar\eta}
\def\hu{{\underline h}}
\def\ho{{\overline h}}
\def\ximin{{\underline\xi}}
\def\ximax{{\overline\xi}}
\def\ximinmin{\underline{\underline\xi}}
\def\ximaxmax{\overline{\overline\xi}}
\def\etaminmin{\underline{\underline\eta}}
\def\etamaxmax{\overline{\overline\eta}}
\def\zetaminmin{\underline{\underline\zeta}}
\def\zetamaxmax{\overline{\overline\zeta}}
\def\etamin{{\underline\eta}}
\def\etamax{{\overline\eta}}
\def\zetamin{{\underline\zeta}}
\def\zetamax{{\overline\zeta}}
\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\ext}{ext}    %extremes 
\DeclareMathOperator{\dist}{dist} 
%\def\xuDLR{x^{u,{\rm{DLR}}}}
\def\XDLR{\overline X^{\,x,\w}}
\def\Xtree{\widehat X^{\,\zeta,\w}}
\def\Xtreen{\widehat X^{\,\zeta,\w,(n)}}
%\def\backpix{{\overleftarrow{\pi}}^x} 
%\def\backpi{{\overset{\small\leftarrow}{\pi}}{}} 
\def\DLR{\mathrm{DLR}}
\newcommand{\siDLR}{\overrightarrow{\DLR}}
\newcommand{\biDLR}{\overleftrightarrow{\DLR}}
\def\CI{\phi}

\def\pici{\pi^{\rm{cif}}}
\def\ker{\kappa}
\def\cid{\xi^*}
\def\Bci{B^*}
\def\Bcil{B^{*,\text\rm{(l)}}}
\def\Bcir{B^{*,\text\rm{(r)}}}
\def\Bbar{\overline B}
\def\Bbarci{\bar B^*}
%\def\cidm{\cid}
\def\cidmin{\underline\xi_{^{\scriptstyle*}}}
\def\cidmax{\overline\xi_*}
\def\ci{{\rm ci}}
\def\Pibar{\overline\Pi}
\def\Pici#1{\Pi^{\ci,\w,#1}}
\def\Picil#1{\Pi^{\ci,\w,\text\rm{(l)},#1}}
\def\Picir#1{\Pi^{\ci,\w,\text\rm{(r)},#1}}
\def\picix{\pi^{x,\ci}}
%\def\varphimin{\varphi^{{\text\rm{(l)}}}}
%\def\varphimax{\varphi^{{\text\rm{(r)}}}}
\def\cidl{\cid^{\text\rm{(l)}}}
\def\cidr{\cid^{\text\rm{(r)}}}
\def\cidlmin{\cidmin^{\text\rm{(l)}}}
\def\cidrmin{\cidmin^{\text\rm{(r)}}}
\def\cidlmax{\cidmax^{\text\rm{(l)}}}
\def\cidrmax{\cidmax^{\text\rm{(r)}}}
%\def\cTl{\cT^{\textrm{(l)}}}
%\def\thetal{\theta_*^{\text\rm{(l)}}}
%\def\thetar{\theta_*^{\text\rm{(r)}}}
%\def\Bcir{\overline B_*}
%\def\Bcil{\underline B_*}


\def\orig{\textit{o}}

\newcommand{\That}{\widehat{T}}
\def\Omtemphat{\widehat\Omega_0}
\def\Ommono{\Omega_{\rm{coc}}} %the Omega on which monotonicity (and other properties?) of cocycles holds
\def\Ommonohat{\widehat\Omega_{\rm{coc}}} %the Omega on which monotonicity (and other properties?) of cocycles holds
\def\Omcont#1{\Omega_{\rm{cont},#1}} %the Omega on which continuity holds at \xi
\def\Omconthat#1{\widehat\Omega_{\rm{cont},#1}} %the Omega on which continuity holds at \xi
\def\Omconstt#1{\Omega_{\rm{tilt},#1}} %the Omega on which h(B) is constant
\def\Omconsthat#1{\widehat\Omega_{\rm{tilt},#1}} %the Omega on which h(B) is constan
\def\Omback#1{\Omega_{#1,\downarrow0}} %the Omega on which the B-tree dies out
\def\OmBus{\Omega_{[\ximin,\ximax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \xi
\def\Ombi{\Omega_{\rm{bi},[\ximin,\ximax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \xi
\def\OmBuszeta{\Omega_{[\zetamin,\zetamax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \zeta
\def\OmBusnice{\Omega_1} %the Omega on which Busemann limits exist on a dense set
\def\OmBusa{\Omega_a} %the Omega on which one force one solution holds 
\def\Omshape{\Omega_{\rm{shape}}} %the Omega on which the shape thms hold
\def\OmBushat{\widehat\Omega_{[\ximin,\ximax]}} %the Omega on which Busemann limit holds
\def\OmBushatzeta{\widehat\Omega_{[\zetamin,\zetamax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits 
\def\OmBusallhat{\widehat\Omega_{\rm{Bus}}} %the Omega on which liminf and limsup bounds hold for Busemann limits for all \xi
\def\OmBusall{\Omega_{\rm{Bus}}} %the Omega on which liminf and limsup bounds hold for Busemann limits for all \xi
\def\Omexist{\Omega_{\rm{exist}}} %the Omega on which directedness of cocycle DLRs holds
\def\Omexistxi{\Omega_{\rm{exist},\xi}} %the Omega on which directedness of cocycle DLRs holds
\def\Omexisthat{\widehat\Omega_{\rm{exist}}} %the Omega on which directedness of cocycle DLRs holds
\def\Omdir{\Omega_{\rm{dir}}} %the Omega on which every DLR is directed
\def\Omdirhat{\widehat\Omega_{\rm{dir}}} %the Omega on which every DLR is directed
\def\OmBusPi{\Omega'_{[\ximin,\ximax]}} %the Omega on which DLR is Busemann for the given \xi
\def\OmBusPihat{\widehat\Omega'_{[\ximin,\ximax]}} %the Omega on which DLR is Busemann for the given \xi
\def\OmBusPiall{\Omega_{\rm{uniq}}} %the Omega on which Busemann limits will hold for all directions at once
\def\OmBusPiallhat{\widehat\Omega_{\rm{uniq}}} %the Omega on which Busemann limits will hold for all directions at once
\def\Omnondeg{\Omega_{\rm{nondeg}}}  %the Omega on which the only non-degenerate DLR solutions are \Pi^{e_i}
\def\OmBhat{\widehat\Omega_B}  %the Omega on which the DLR solution corresponding to B is directed
%\def\OmB{\Omega_B}  %the Omega on which the DLR solution corresponding to B is directed
%\def\Omreg{\Omega_{\rm{reg}}} % the Omega on which regular conditional probabilities are supported on the projection
\def\Omcif{\Omega_{\rm{cif}}} % the Omega on which regular conditional probabilities are supported on the projection
\def\Omnonuniq{\Omega_{\rm{ex}}} %the Omega on which Usetnonuniq does not intersect linear segments and includes non-diff points
\def\Omeihat{\widehat\Omega_{e_1,e_2}}


\def\WLLN{WLLN$_\xi$}
\def\SLLN{SLLN$_\xi$}
\def\proj{\pi}
\def\gDLR{\mathrm{gDLR}}
\def\cgDLR{\mathrm{cgDLR}}

\allowdisplaybreaks
%\allowdisplaybreaks[3]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environment definitions go here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{formal}[theorem]{Critical point derivation}
%\newtheorem{experiment}[theorem]{Experimental Result}
%\newtheorem{clam}[theorem]{Claim}
%\newtheorem{condition}[theorem]{Condition}


%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{xca}[theorem]{Exercise}
%\newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{conj}[theorem]{Conjecture}
%
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
%\newenvironment{remarks}{\begin{remark}\normalfont}{\end{remark}}
%
%\newtheorem{quest}{Question}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%C: Single counter environments with triangles.
\newtheorem{mainCounter}{MainCounter}[section]

\newtheorem{lemma}[mainCounter]{Lemma}
%\AtBeginEnvironment{lemma}{%
%  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
%}
%\AtEndEnvironment{lemma}{\popQED\endremark}
%
\newtheorem{theorem}[mainCounter]{Theorem}
%\AtBeginEnvironment{theorem}{%
%  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
%}
%\AtEndEnvironment{theorem}{\popQED\endremark}


\newtheorem{itheorem}[mainCounter]{Informal Theorem}

\newtheorem{proposition}[mainCounter]{Proposition}
%\AtBeginEnvironment{proposition}{%
%  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
%}
%\AtEndEnvironment{proposition}{\popQED\endremark}

\newtheorem{corollary}[mainCounter]{Corollary}
%\AtBeginEnvironment{corollary}{%
%  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
%}
%\AtEndEnvironment{corollary}{\popQED\endremark}


\numberwithin{equation}{section}

\newtheorem{definition}[mainCounter]{Definition}
%\AtBeginEnvironment{definition}{%
%  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
%}
%\AtEndEnvironment{definition}{\popQED\endremark}

\newtheorem{condition}[mainCounter]{Condition}

\theoremstyle{remark}
\newtheorem{remark}[mainCounter]{Remark}
\AtBeginEnvironment{remark}{%
  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
}
\AtEndEnvironment{remark}{\popQED\endremark}
\newtheorem{example}[mainCounter]{Example}
\AtBeginEnvironment{example}{%
  \pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}%
}
\AtEndEnvironment{example}{\popQED\endremark}




%%%%%%%   the BEST  Timo macros (2018-01-19--)  %%%%%%%%

\newcommand{\nn}{\nonumber}

\DeclareMathOperator{\hull}{\overline{\text{co}}}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\bd}{bd}

\DeclareMathOperator{\sign}{sign} 
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\card}{card}
%\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\trace}{trace}
%\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\Var}{\mathbb Var}
  \DeclareMathOperator{\Cov}{Cov}  
  \DeclareMathOperator{\conv}{co}   %convex hull  


%\DeclareMathOperator{\proj}{Proj}
%\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\aff}{aff}   %affine hull  
\DeclareMathOperator{\effdom}{dom}   %eff domain 
\DeclareMathOperator{\id}{id}


\font \mymathbb = bbold10 at 11pt
\newcommand{\ind}{\mbox{\mymathbb{1}}}
%\def\ind{\mathbf{1}}
\def\deq{\overset{d}=} 
\def\dto{\overset{d}\to} 
\def\qedex{\hfill$\triangle$} 
\def\qedrm{\hfill$\triangle$} 
\def\iff{\Longleftrightarrow}      \def\iiff{\ \Longleftrightarrow \ }
\def\implies{\Longrightarrow}   \def\iimplies{\ \Longrightarrow\ }
\def\rimplies{\Longleftarrow}

\newcommand{\bD}{\mathbb{D}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cIhat}{\widehat{\mathcal{I}}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cKhat}{\widehat{\mathcal{K}}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cThat}{\widehat{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\def\Z{\bbZ} 
\def\R{\bbR} 
\def\N{\bbN} 

\def\Xw{X}  %another letter for a weight 
\def\Yw{Y}  %another letter for a weight 
\def\Ywch{\wc\Yw}  %another letter for a weight 

 \def\evec{e}   %%% use this if we do not want boldface e_1 and e_2. 
% \def\evec{\mathbf{e}} 
  \def\uvec{\mathbf{u}}\def\vvec{\mathbf{v}}
   \def\avec{\mathbf{a}} \def\bvec{\mathbf{b}}
%  \def\hvec{\bm{h}}      
  \def\hvec{\mathbf{h}}   
  \def\ivec{\mathbf{i}} 

\def\kvec{\mathbf{k}}  \def\mvec{\mathbf{m}}   \def\nvec{\mathbf{n}}
 \def\pvec{\mathbf{p}}
\def\xvec{\mathbf{x}}
\def\yvec{\mathbf{y}}
\def\zvec{\mathbf{z}}
\def\wvec{\mathbf{w}}
\def\Jvec{\mathbf{J}}
\def\Xvec{\mathbf{X}} \def\Yvec{\mathbf{Y}}  \def\Zvec{\mathbf{Z}} \def\thvec{\boldsymbol{\theta}}

\def\xhat{\widehat x}
\def\zhat{\widehat z}
\def\xbar{\overline x}
\def\absorb{\triangleleft}

\def\timonote#1{{\color{violet}{(T: #1)}}}
\def\firasnote#1{{\color{orange}{(F: #1)}}}
\def\chrisnote#1{{\color{olive}{(C: #1)}}}
\def\mathnote#1{{\color{red}{(#1)}}}
\def\textnote#1{{\color{blue}{(#1)}}}
\def\textargument#1{{\color{brown}{(#1)}}}
\def\later#1{{\color{cyan}{(#1)}}}

\def\E{\bbE}
\def\Ehat{\widehat\bbE} %% environment measure 
\def\Ebar{\overline\bbE} %% environment measure 
\def\P{\bbP} %% environment measure 
\def\Phat{\widehat\bbP} %% environment measure 
\def\Pbar{\overline\bbP} %% environment measure 

 \def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline} \def\wc{\widecheck}

\def\Bus#1{B^{#1}} 
\def\rBus#1{\wt B^{#1}}
\def\wtBus#1{\wt B^{#1}}
\newcommand\Busv[3]{\overline B^{\,#1,#2}_{#3}}

\def\RW{S}
\def\ZRW{Z}
\def\Zero{R}
\def\Zerobar{\overline\Zero}

%%%%%%%   Random measures with superscript "Bus" 
%\def\Bpp{\mathbf{n}^{\text{\rm Bus}}}  %  \Bpp = Busemann pt process of jump locations 
%\def\Bppa{{\boldsymbol\nu}^{\text{\rm Bus}}}   %  \Bppa = Busemann pt process of jump locations and jump sizes
%\def\Bppb{{\boldsymbol\mu}^{\text{\rm Bus}}}   %Busemann measure on edge k 
%\def\Bmeas{\mu^{\text{\rm Bus}}} 
%\def\Bmeasb{\boldsymbol{\nu}^{\text{\rm Bus}}} 
%\def\Bmm{m^{\text{\rm Bus}}}   %mean Busemann measure 

%%%%%  These random measures without superscript "Bus" 
\def\Bpp{\mathbf{n}}  %  \Bpp = Busemann pt process of jump locations 
\def\Bppa{{\boldsymbol\nu}}   %  \Bppa = Busemann pt process of jump locations and jump sizes
\def\Bppavar{\nu}   %  \Bppa = Busemann pt process of jump locations and jump sizes
\def\Bppb{{\boldsymbol\mu}}   %Busemann measure on edge k 
\def\Bmeas{\mu} 
\def\Bmeasb{\boldsymbol{\nu}} 
\def\Bmm{\lambda}   %mean Busemann point measure 
\def\umeas{u}   %measure of point locations of a purely atomic measure 

%\def\Hgraph{\cH}  %a graph 
\newcommand\Hgraph[1]{\mathcal{H}_{#1}}
\def\zclus{\bfK}    %notation for the backward cluster of z 
\def\cifset{\bfD}  %set of vertices with asymptotic cif direction in a set 
\def\xisim{\,\overset\xi\sim\,}    %equivalence relation  
%\def\zesim{\,\overset{[\zeta, \eta]}\sim\,}    %equivalence relation 
\def\zesim{ \overset{[\zeta, \eta]}\sim }    %equivalence relation without extra space

\def\depa{B}  %% departure processes from queues, also the generic variable for Busemanns in the description of the joint distribution. 
\def\serv{w}     %% service variables 

\def\level{\bbL}     %%%% levels on lattice 


 

\newcommand\bnearrow{{\raisebox{1pt}{\scaleobj{0.5}{\mathbf\nearrow}}}}   %% \nearrow for a superscript so it doesn't look ridiculously big 
    
\def\caY{\cY^{\bnearrow}}  % a space of ordered n-tuples 
\def\caaY{\cY^{\bnearrow\!\bnearrow}}  % a space of ordered n-tuples 
\def\paramb{\tau}   %% needed a parameter -- not sure what a good letter choice is. 
   
\def\gdirv{\xi}    %geodesic direction 
\def\gdirc{\xi\cdot\evec}  %coordinate of a geodesic direction 

\def\Dop{D}    %%% D operator for departure process 
\def\Rop{R}  %% check weights or time in the back of the queue  
\def\Sop{S}    %%% S operator for sojourn time process 
\def\Daop{\cD}   %%n"bigger" operators 
\def\Taop{\cT}
\def\Saop{\cS} 
\def\rDop{{\overleftarrow\Dop}}    %%% reverse D operator for departure process 
\def\rRop{{\overleftarrow\Rop}}  %% check weights or time in the back of the queue  
\def\rSop{{\overleftarrow\Sop}}    %%% S operator for sojourn time process 
\def\fDop{{\overrightarrow\Dop}}    %%% forward D operator for departure process 
\def\fRop{{\overrightarrow\Rop}}  %%   forward
\def\fSop{{\overrightarrow\Sop}}    %%%   forward
\def\refl{\rho}   % reflection 

\def\OFP{(\Omega, \cF, P)}    \def\OF{(\Omega, \cF)}  
\def\OSP{(\Omega, \mfS, \P)}

   \newcommand{\lzb}{\llbracket}   %left Z bracket  
\newcommand{\rzb}{\rrbracket}   %right Z bracket 

\def\indep{\ \ \,{\raisebox{-1pt}{\text{\begin{rotate}{90}$\models$\end{rotate}}}}\ \, }  %independent random variables 
\def\nindep{\ \ \,{\raisebox{-1pt}{\text{\begin{rotate}{90}$\nvDash$\end{rotate}}}}\ \, }   %not independent random variables 

\newcommand\abullet{{\scaleobj{0.6}{\bullet}}}  %%%% smaller bullet to use inside functions 
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.6}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-1pt}{\scaleobj{0.5}{\bullet}}}} %%  for subscript paths x_\brbullet   need negative raise 
\newcommand\cbullet{{\raisebox{1pt}{\scaleobj{0.6}{\bullet}}}}   %% looks good on Busemann process \Bus^\cbullet  as a superscript  

\newcommand\dbullet{{\scaleobj{0.7}{\bullet}}}   % same as \bbullet but without shift up

\newcommand\bcdot{{\scaleobj{1.8}{\cdot}}}
\newcommand\acdot{{\raisebox{-1.5pt}{\scaleobj{1.6}{\cdot}}}}  %%dot inside function 

%%%%%%%%   End Timo's macros %%%%%%%%%

%\usepackage{filemod}   
%\usepackage[short,nodayofweek,level,12hr]{datetime}   %%% clash

\overfullrule=5pt


%%%%%%   Timo added 2020-11-30  --->  
\def\pathsp{\mathbb{X}}   %path space
\def\finpathsp{\mathbb{X}^{\rm{fin}}}   %path space
\def\pathspbi{\mathbb{X}^{\rm{bi}}}
\def\pathsa{\mathcal{X}}   %path sigma algebra
\newcommand\ptail{\mathcal{X}_{\textup{tail}}}


\def\zevec{\mathbf 0}

\def\tsp{\hspace{0.5pt}}  %this is sometimes a good spacing in formulas when \, is too large 
\def\tspa{\hspace{0.7pt}}
\def\tspb{\hspace{0.9pt}}
\def\tspc{\hspace{1.1pt}}

\def\pathsp{\mathbb{X}}   %path space  
\def\pawgt{G}  %path weight 
\def\parng#1#2{#1\hspace{0.6pt}{\boldsymbol:}\hspace{0.3pt}#2}  %path range 



\def\coal{\curlywedgeuparrow}  %%%% coalescence relation. 
\newcommand{\ncoal}{%
\tikz[baseline, inner sep=0.5pt] \node[strike out,draw,anchor=text,inner sep=0pt,text=black]{$\coal$};} %Not coalesce. Requires \usetikzlibrary{shapes.misc}

\newcommand\coalpt{\mathbf{z}} %Coalescence point
\newcommand\Cset{C} %coalescence set

 \def\Vvv{{\rm\mathbb{V}ar}}  \def\Cvv{{\rm\mathbb{C}ov}} 
 
 \def\ind{\mathbf{1}}    %% T's favorite indicator notation -- change it if you want!   
 
 \def\viiva{\hspace{.7pt}\vert\hspace{.7pt}}
\def\bviiva{\hspace{.7pt}\big\vert\hspace{.7pt}}   %% big viiva, use with \She\bigl( ... \bviiva ... \bigr) 
\def\Bviiva{\hspace{.7pt}\Big\vert\hspace{.7pt}} 

%%%%%%%%%%%%%   oriented percolation   
\def\opc{\vec p_c}  
\def\cla{\cO} 
\def\clb{\cO} 
%\def\pc{\vec p_c}
\def\etamin{{\underline\eta}}
\def\etamax{{\overline\eta}}

\def\badevent{R}   \def\badeventA{A}     %% generic letter for bad events in lemmas  2025-01-27  

\def\apreceq{\preceq_a}
\def\aprecneq{\precneq_a}
\def\asucceq{\succeq_a}
\def\asuccneq{\succneq_a}

 %%%%%%  end T additions %%%%%%%%

\def\Bus{B} %generalized Busemann
\def\Busgeo{A} %geodesic Busemann
\def\Buss{\Busgeo} %Busemann of the geodesic x^s
\def\Bush{\Bus} %generalized Busemann with tilt h
\def\Bushtmp{\overline\Bus} %generalized Busemann with tilt h
\def\Busxi{\Bus} %generalized Busemann with direction \xi (probably don't use these?)
\def\Busa{\Bus} 

\def\hhB{\hvec} 

\def\wg{\eta}
 \def\wgtil{\tilde\eta}

\def\Lpp{L}    %% LPP introduced 2022-05-17  

\def\nojump{{\rm NJ}}      % no-jump event 
\def\ranvar{X}           %% a random variable 
\def\cube{\bD}   %% cube or \ell^\infty ball 

\newcommand\map{p}
\newcommand\jumps{\cJ}
\newcommand\edge{S}
\newcommand\tie{\mathfrak t}
\newcommand\tiemin{\underline{\mathfrak t}}
\newcommand\tiemax{\overline{\mathfrak t}}
\newcommand\edgehat{\wh\edge}
\newcommand\cdfpi{{\boldsymbol{\pi}}}
\newcommand\leb{\cL}
\newcommand\pihat{\wh\pi}
\newcommand\gammahat{\wh\gamma}
\newcommand\supgeod{\overline\gamma}
\newcommand\supgeodst{\gamma}

%%%%%%%%%%%%%%%%%%
%Chris Macros
%Isolated geodesic sets
\newcommand\LI{\textup{LI}} %Left isolated
\newcommand\RI{\textup{RI}} %Right isolated
\newcommand\I{\textup{I}} %Isolated geodesics
\DeclareMathOperator\Gr{Gr}
\newcommand\PrOm{\textup{Pr}_{\Omega}}
\newcommand\PrOmB{\textup{Pr}_{\Omega\times(0,\infty)}}

%Event on which the Busemann cocycle is extremal
\newcommand\Omhatext{\Omhat_{\textup{B,ext}}}

%CDF measures
\newcommand\cdfm{\mathbf{m}}


\newcommand\Geof{\mathfrak{G}} %Set of all finite geodesics.

%Partition functions, pathspace, and polymer measures
\newcommand\Path[2]{\bbX_{#1}^{#2}}
\newcommand\PF[2]{\textup{\textup{Z}}_{#1,#2}} %The polymer partition function.
\newcommand\FE[2]{\textup{\textup{F}}_{#1,#2}} %The passage
\newcommand\poly[2]{\textup{\textup{Q}}_{#1,#2}}

%Concatenation of paths
\newcommand\concat{\diamond}

%Mesaureson paths
\newcommand\mD{\mathfrak{M}} %Dense subset of the space of measures on paths

\newcommand\Skor{\textup{D}_{\textup{LCRL}}}
\newcommand\aabullet{{\raisebox{1.3pt}{\hspace{0.6pt}\scaleobj{0.55}{\bullet}\hspace{0.75pt}}}}  %%%% smaller bullet to use inside
\DeclareMathOperator{\uE}{E}

\newcommand\dy{\textup{D}} %Dyadic intervals at scale m are \dy_m.
\DeclareMathOperator{\dya}{D} %D_{k,m} = []
\newcommand\dyatup{\mathbf{D}} %$2^n$-tuple of dyadic intervals
\newcommand\edy{\mathcal{E}} %$\edy_{n}(\dyatup)$ is the collection of extremal Gibbs measures which assign probabilities in a given $2^n$-tuple of dyadic intervals at scale $m$.
\newcommand\Dmeas{\mathfrak{D}}
